Muckenhoupt's $(A_p)$ condition and the existence of the optimal martingale measure

In the problem of optimal investment with utility function defined on $(0,\infty)$, we formulate sufficient conditions for the dual optimizer to be a uniformly integrable martingale. Our key requirement consists of the existence of a martingale measure whose density process satisfies the probabilistic Muckenhoupt $(A_p)$ condition for the power $p=1/(1-a)$, where $a\in (0,1)$ is a lower bound on the relative risk-aversion of the utility function. We construct a counterexample showing that this $(A_p)$ condition is sharp.

==> style.tex <==
% Packages

\usepackage{amsthm} \usepackage{amsmath} \usepackage{amsfonts}
\usepackage{amssymb} \usepackage{latexsym} \usepackage{enumerate}
\usepackage{mathrsfs}
\usepackage[numbers]{natbib}
\usepackage[colorinlistoftodos, textwidth=4cm, shadow]{todonotes}

\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

% Theorems and similar

\theoremstyle{plain}%
\newtheorem{Theorem}{Theorem}[section] %
\newtheorem{Corollary}[Theorem]{Corollary}%
\newtheorem{Lemma}[Theorem]{Lemma} %
\newtheorem{Proposition}[Theorem]{Proposition} %

\theoremstyle{definition}%
\newtheorem{Assumption}[Theorem]{Assumption}%
\newtheorem{Definition}[Theorem]{Definition}%
\newtheorem{Example}[Theorem]{Example} %

\theoremstyle{remark}%
\newtheorem{Remark}[Theorem]{Remark} %

% Useful commands

\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\Ap}[1]{(A_{#1})}
\newcommand{\Rq}[1]{(R_{#1})}
\newcommand{\braces}[1]{\left\lbrace{#1}\right\rbrace}
\newcommand{\descr}[2]{\left\lbrace{#1}:\; #2 \right\rbrace}

% Conditional expectation: measure, time, RV
\newcommand{\cE}[3]{\mathbb{E}^{#1}\left[\left.#3\right\lvert\mathcal{F}_{#2}\right]} 
\newcommand{\E}[2]{\mathbb{E}^{#1}\left[#2\right]} 
\newcommand{\EP}[1]{\E{}{#1}}
\newcommand{\cEP}[2]{\cE{}{#1}{#2}}
\newcommand{\EQ}[1]{\E{\mathbb{Q}}{#1}}
\newcommand{\cEQ}[2]{\cE{\mathbb{Q}}{#1}{#2}}
\newcommand{\C}{C}

\newcommand{\bmo}{\mathrm{BMO}}
\newcommand{\bmonorm}[1]{\lVert#1\rVert_{\bmo} } %
\newcommand{\Ebmo}{\mathcal{E}(\bmo)}
\newcommand{\seq}[1]{$\left(#1^n\right)_{n\geq 1}$}
\newcommand{\set}{\triangleq}
\newcommand{\ip}[2]{\left\langle
    #1,#2 \right\rangle}
\newcommand{\qv}[1]{\left\langle
    #1\right\rangle}
\newcommand{\ind}[1]{1_{\braces{#1}}}
\newcommand{\setind}[1]{1_{#1}}
\newcommand{\map}[3]{#1:\; #2 \rightarrow #3} %1=name, 2=arg_domain, 3=val_domain
\newcommand{\mtext}[1]{\;\text{#1}\;}
\newcommand{\mmtext}[1]{\quad\text{#1}\quad} 
\newcommand{\norm}[1]{\lVert#1\rVert} %

% Environments

\newcommand{\envspace}{\vspace{2mm}}
\newenvironment{ToDo}{\envspace
  \noindent {\textbf{Things to do:}}  \sf}{\envspace}


